A Black Swan Hypothesis: The Role of Human Irrationality in AI Safety

Black swan events are statistically rare occurrences that carry extremely high risks. A typical view of defining black swan events is heavily assumed to originate from an unpredictable time-varying environments; however, the community lacks a comprehensive definition of black swan events. To this end, this paper challenges that the standard view is incomplete and claims that high-risk, statistically rare events can also occur in unchanging environments due to human misperception of their value and likelihood, which we call as spatial black swan event. We first carefully categorize black swan events, focusing on spatial black swan events, and mathematically formalize the definition of black swan events. We hope these definitions can pave the way for the development of algorithms to prevent such events by rationally correcting human perception.

==> files/Dummy_3.tex <==
% \section{How misperception raise \ours}

% This section provides a case study to fully support Hypothesis \ref{hyp1} before defining \ours. Subsection explains how a misperception on the event probability, the humans can make irrational decision making and lead to a black swan in a stationary environment.
% \subsection{
% Revising Von Neumann-Morgenstern Theory to Account for Human Irrationality}
% \label{subsec:}
%  Von Neumann–Morgenstern (VNM) theory explains how humans can make rational decisions under uncertainty. The theory is built upon four axioms: completeness, transitivity, continuity, and independence (See Appendix). However, in order to explain the irrationality of human decision-making, we claim that the \emph{continuity} and \emph{independence} axioms need to be revised, and revised axioms provide a sound ground on the $\textsc{s- black swan}$ emergence. We explain VNM axioms and those revised versions in the MDP context as follows. \cp{I might delete every part except the first sentence in front of this comment. so start with the next sentence. } Suppose, $N$ outcomes (states) $\cS = \{ s^{(1)},s^{(2)},\cdots,s^{(N)} \}$ and have action space $\cA$. We define action $a \in \cA$ as returning $s^{(j)}$ with probability $p^{(j)}_{a} \geq 0$ and denote it as $\sum_{j=1}^{N} p^{(j)}_{a} s^{(j)}$. VNM theory defines that $s^{(i)}$ is preferred over (or equally preferred) $s^{(j)}$ if $g(s^{(i)}) > g(s^{(j)})$ or $(g(s^{(i)}) = g(s^{(j)}))$ holds where $g$ is a utility function, and also defines $a^{(i)}$ is preferred over (or equally preferred) $a^{(j)}$ if $\sum_{k=1}^{N} p_{ik} g(s^{(k)}) > \sum_{k=1}^{N} p_{jk}  g(s^{(k)})$ (or $\sum_{k=1}^{N} p_{ik} g(s^{(k)}) = \sum_{k=1}^{N} p_{jk}  g(s^{(k)})$) holds. The continuity and independence axioms of VNM theory are given as
 
%  % For $a^{(1)},a^{(2)}$, and $a^{(3)}$, we suppose $a^{(1)}$ returns an outcome $s^{(1)}$ with probability $p$ and $s^{(3)}$ with probability $1-p$ and action $a^{(2)}$ returns an outcome $s^{(2)}$ with probability $p$ and $s^{(3)}$ with probability $1-p$, and action $a^{(3)}$ returns an outcome $s^{(2)}$ with probability $1$. \cp{so do we assume 3 action 3 state? I think this might be not appropriage as we are generally explaining VNM. We need separate paragraph. }  

% \begin{axiom}[Independence and Continuity axioms of VNM theory]
% \quad
%     \begin{itemize}
%     \item \textbf{Independence.} If $s^{(1)}$ is preferred to $s^{(2)}$, and a event probability $p \in [0,1]$, then action $p s^{(1)} + (1-p) s^{(n)}$ is preferred to action $p s^{(2)} + (1-p) s^{(n)}$ for any $ n \in [N]$.
%     \item \textbf{Continuity.} If $s^{(1)}$ is preferred to $s^{(2)}$ and $s^{(2)}$ is preferred to $s^{(3)}$, there exists a event probability $p \in [0,1]$ such that action $1 \cdot s^{(2)}$ is considered equally preferable to action $p s^{(1)} + (1-p) s^{(3)}$.
% \end{itemize}
% \label{axiom1}
% \end{axiom}

% \cp{actually we do not know what is the meaning of independence and continuity generally, so I actually did not get both of them. }\hl{revised. Please check.}  The Independence Axiom ensures that a decision-maker's preference between two outcomes remains consistent even when both are part of a mixed gamble with a third outcome, unaffected by the presence of identical alternatives. The Continuity Axiom ensures that a decision-maker's preferences are smooth and consistent, allowing for indifference between a certain outcome and a gamble involving more and less desirable outcomes without abrupt shifts in preference. However, Axiom \ref{axiom1} does not fully capture the decision-making process in real-world scenarios where humans often make irrational choices. To address this, we introduce a subjective probability through a probability distortion function $w$ from Assumption \ref{asp:Weight function}. By incorporating this function into the Axiom \ref{axiom1}, we propose the following revised version. For notation simplicity, we denote action $a^{(i)}$ as 
% \begin{axiom}[Revised VNM Axioms in the MDP Context to Explain Human Irrationality] \quad
%      \begin{itemize}
%          \item \textbf{Subjective Dependence.} 
%          If there exists $p$ that satisfies $w(p)=0$ for any two actions  \(p s^{(1)} + (1-p) s^{(n)}\) and \(p s^{(2)} + (1-p) s^{(n)}\), the human perceives those two actions are equally preferable, however, in the real world, action $p s^{(1)} + (1-p) s^{(n)}$ is preferrable to $p s^{(2). } + (1-p) s^{(n)}$. That is, $s^{(n)}$ does not work as an ``independent factor' as expected but instead inversely affects the preference, misleading the decision-maker.
         
%          ===============\\
%          Humans choose between two actions, \(p s^{(1)} + (1-p) s^{(n)}\) and \(p s^{(2)} + (1-p) s^{(n)}\), by comparing their perceived utility values, i.e., \(w(p) g(s^{(1)}) + (1-w(p)) g(s^{(n)})\) and \(w(p) g(s^{(2)}) + (1-w(p)) g(s^{(n)})\). In contrast, a rational action choice in the real world would involve comparing the true utility values \(p g(s^{(1)}) + (1-p) g(s^{(n)})\) and \(p g(s^{(2)}) + (1-p) g(s^{(n)})\) for any \(n \in [N]\).

%          \item \textbf{Subjective Discontinuity.} 
%          Humans perceive two actions, \(1 \cdot s^{(2)}\) and \(p s^{(1)} + (1-p) s^{(3)}\), as not equally preferable if $w(p) \neq p$. However, in the real world, \(1 \cdot s^{(2)}\) is considered equally preferable to \(p s^{(1)} + (1-p) s^{(3)}\). That is, the action set $\{ 1 \cdot s^{(1)}, 1 \cdot s^{(2)}, 1\cdot s^{(3)}\}$ can be exactly bisected by "preferable" or "Non-preferable" to \(p s^{(1)} + (1-p) s^{(3)}\) , and there does not exists exact equable point. 
         
         
         
         
%          ================\\
%          Humans perceive two actions, \(1 \cdot s^{(2)}\) and \(p s^{(1)} + (1-p) s^{(3)}\), as not equally preferable if $w(p) \neq p$. However, in the real world, \(1 \cdot s^{(2)}\) is considered equally preferable to \(p s^{(1)} + (1-p) s^{(3)}\). This implies that humans might identify another action \(1 \cdot s^\prime \in \cA\) such that its utility value equals \(w(p) g(s^{(1)}) + (1-w(p)) g(s^{(3)})\), where \(s^{(1)}\) is preferred over \(s^\prime \in \cS\) and \(s^\prime\) is preferred over \(s^{(3)}\).
%      \end{itemize}
% \label{axiom2}
% \end{axiom}

% \cp{At least we need to explain what is the meaning of independence and continuity (intuitively)} \hl{I got it. I'll come back later on} We now further illustrate the emergence of \ours due to subjective probability with the following two examples. To set the stage, Example \ref{ex1} demonstrates how \emph{subjective continuity} can lead to potential risk in decision-making.

% \begin{example}[How subjective probability leads to risky decision]
%     Suppose utility value of three states $s^{(1)},s^{(2)},$ and $s^{(3)}$ as $g(s^{(1)})= -1, g(s^{(2)})=-1000, g(s^{(3)})=1000$, where \( s^{(2)} \) is an extremely risky outcome.  Now suppose that the \( a^{(1)} \) returns \( s^{(2)} \) with \( 50.05\% \) and \( s^{(3)} \) with \( 49.95\% \) and $a^{(2)}$ returns $s^{(1)}$ with probability $1$. Then, in the real world, action \( a^{(1)} \) and \( a^{(2)} \) return the same utility value as \( g(s^{(2)}) \cdot p_2 + g(s^{(3)}) \cdot p_3 = -1000 \cdot 0.5005 + 1000 \cdot 0.4995 = -1 \) and $g(s^{(1)}) \cdot p_1 = 1 \cdot (-1) =-1$. However, if human perceive that \( a^{(2)} \) returns \( s^{(2)} \) with \( 50.01\% \) and \( s^{(3)} \) with \( 49.99\% \), then $a^{(4)}$ returns the value \( -1000 \cdot 0.5001 + 1000 \cdot 0.4999 =-0.2 \), and thus determine an optimal policy as choosing  \( a^{(2)}  \).
%     \label{ex1}
% \end{example}
%     In reality, choosing between choice \( a^{(2)} \) and \( a^{(4)} \) does not matter since both provide the same utility value, but choosing choice \( a^{(2)}\) is actually more risky than choice \( a^{(4)} \) since choice \( a^{(2)} \) contains the high-risk outcome \( B \). \cp{I guess this is just a CPT example. Why this is related to blackswan? is it a new example? } \hl{check just right before sentence of your comment. I agree that Example 1 is similar to CPT that this one highlights irrational decision-making can also related to risky decision that the human have not expected.}\cp{At least we need to explain HOW different this example is from original (or popular) CPT example. I did not get the different part. } Now, we go beyond irrational risky decisions and explain how subjective probability raises \ours by underestimating the low event probabiltiy in the following example.

% \begin{example}[How \emph{subjective independence} raise \ours ]
%     Continuing from Example \ref{ex1}, consider choosing between two actions \( a^{(3)} \) and \( a^{(4)} \) where \( a^{(3)} \) returns \( 0.001\% \) of \( s^{(1)} \) and \( 99.999\% \) of \( s^{(3)} \), and  \( a^{(4)} \) returns \( 0.001\% \) of \( s^{(2)} \) and \( 99.999\% \) of \( s^{(3)} \). Through several trials, due to the extreme rarity of occurrence of \( s^{(1)} \) or \( s^{(2)} \), regardless of choosing \( a^{(1)} \) or \( a^{(2)} \), humans perceive that both return the same utility value of \( g(s^{(3)}) = 1000 \), which can be interpreted as \( w(0.001\%) = 0\% \) and \( w(99.999\%) = 100\% \), and decide their optimal policy is random sampling. However, over time, humans have a probability of encountering \( s^{(2)} \) with a probability of \( 0.0005\% \), which is a black swan.
%     \label{ex2}
% \end{example}

% Examples \ref{ex1} and \ref{ex2} clearly shows that mispercpetion on event probability leads to irrational risk decision and further emergence of black swans.
% \subsection{The Emergence of \ours Events in Sequential Decision Making}
% Now, we go further. Let's see how \ours emerges in sequential decision making. We start from bandit case. For given $(s,a) \in \cS \times \cA$, let us assume function $u$ distorts reward $R_t(s,a)$ and function $w$ distorts the transition probability $P_t(s^\prime | s,a)$ at time $t$ where $s^\prime$ is the next state where Assumptions \ref{asp:Utility function} and \ref{asp:Weight function} are still hold. For this section, We say MDP which is distorted by function $u,w$ as distorted MDP.

% \subsubsection{Case 1. Contextual Bandit ($T=1$)}
% We begin with a simple case where the decision horizon is \( T = 1 \), commonly referred to as a contextual bandit (\cite{lattimore2020bandit}). Surprisingly, in this setting, the human optimal policy coincides with the real-world optimal policy. This is somewhat counterintuitive, as Examples \ref{ex1}, \ref{ex2} suggest that human decision-making often exhibits irrationality.

% \begin{theorem}[One-step Optimality Deviation]
%     If \( T=1 \), then the optimal policy from the MDP aligns with the optimal policy of the distorted MDP.
%     \label{thm:one step perceived optimal policy}
% \end{theorem}

% An important insight from Theorem \ref{thm:one step perceived optimal policy} is that when decisions are not sequential, the typical distortions in human perception do not affect the alignment with the optimal policy of the real world, suggesting that human irrationality is less influential in a single-step decision-making setting. This is further explained in the following remark.

% \begin{remark}
%     Continuing from Example \ref{ex1}, the order of perceived rewards does not change as \( u^-( g(r(s^{(1)}))) < u^-( g(r(s^{2)})) < u^+( g(r(s^{(3)}))) \), since \( u^- \) is a non-decreasing convex function and \( u^+ \) is a non-decreasing concave function.
%     \label{rmk:1}
% \end{remark}

% \subsubsection{Case 2. $|\mathcal{S}|=2$ when $T >1$}
% Now, let us consider the simplest case where $T > 1$ where $|\mathcal{S}|=2$. Surprisingly, the result that optimality does not deivate still holds similar to Theorem \ref{thm:one step perceived optimal policy}.

% \begin{theorem}[Multi-step human optimal policy]
%     If $|\mathcal{S}|=2$, then the optimal policy from the MDP also aligns with the optimal policy of the distorted MDP for all $t \in [T]$.
%     \label{thm:Multi step perceived optimal policy}
% \end{theorem}

% Theorem \ref{thm:Multi step perceived optimal policy} may seem counterintuitive. However, a heuristic analysis suggests that with only two states in the state space, the actions do not introduce significant variability in randomness. Essentially, if an action introduces randomness, it would likely affect both states $s_{0}$ and $s_{1}$ similarly if the action leads to a nondeterministic next state. As a result, every action yields the same set of possible next states, reducing the problem to a simple comparison between the two states. This observation implies that in scenarios with a smaller state space, irrational beliefs (based on false perceptions) do not lead to deviations from the optimal policy. We can also interpret this result to mean that when $|\cS|$ is small, sequential decision-making problems are relatively \emph{simple}, allowing humans to consistently identify the optimal action in the real world.


% \subsubsection{Case 3. $|S|=3$ when unbiased reward perception}
% We consider the hypothetical scenario where \( u(R_t(s,a)) = R_t(s,a) \) holds for $\forall (s,a)$, indicating that humans have an unbiased perception of their reward.

% \begin{theorem}[Two step optimal decision when $|\cS|=3$]
%     Given any state space $\cS$ where $|\mathcal{S}|=3$ and a decision horizon $T=2$, there exists a $\{ P_t\}_{t=1}^T, \{ R_t\}_{t=1}^T$ such that the optimal policy of MDP differs from that of distorted MDP.
%     \label{thm:Two step optimal decision}
% \end{theorem}

% Theorems \ref{thm:one step perceived optimal policy}, \ref{thm:Multi step perceived optimal policy}, and \ref{thm:Two step optimal decision} illustrate that the discrepancy between human and optimal decision making increases as the complexity of the environment increases ($\cS$) or as the decision sequence ($T$) lengthens for any \( w \) function.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

